Unifying notions of pasting diagrams

In this work, we relate the three main formalisms for the notion of pasting diagram in strict $\omega$-categories: Street's parity complexes, Johnson's pasting schemes and Steiner's augmented directed complexes. In the process, we show that the axioms of parity complexes and pasting schemes are not strong enough for them to correctly represent pasting diagrams, and we do so by providing a counter-example. Then, we introduce a new formalism, called torsion-free complexes, which aims at encompassing the three other ones. We prove its correctness by providing a detailed proof that an instance induces a free $\omega$-category. Next, we prove that the three other formalisms can be embedded in some sense in the new one. Finally, we show that there are no other embedding between these four formalisms.

==> Makefile <==
PDFLATEX=pdflatex
ARXIV_OUT=arxiv_temp
ARXIV_REMOVED=notes.org

all: fast

fast:
	$(PDFLATEX) '\let\ifdebugmode\iffalse\let\ifhs\iffalse\input{article}'

biber:
	biber article

# SF: Higher Structures version
hs:
	$(PDFLATEX) '\let\ifdebugmode\iffalse\let\ifhs\iftrue\input{article}'
	biber article
	$(PDFLATEX) '\let\ifdebugmode\iffalse\let\ifhs\iftrue\input{article}'
	$(PDFLATEX) '\let\ifdebugmode\iffalse\let\ifhs\iftrue\input{article}'
	cp article.pdf article-release.pdf

arxiv:
	$(PDFLATEX) '\let\ifdebugmode\iffalse\let\ifhs\iffalse\input{article}'
	biber article
	$(PDFLATEX) '\let\ifdebugmode\iffalse\let\ifhs\iffalse\input{article}'
	$(PDFLATEX) '\let\ifdebugmode\iffalse\let\ifhs\iffalse\input{article}'
	cp article.pdf article-arxiv.pdf

arxiv_archive:
	rm -rf ${ARXIV_OUT}
	mkdir ${ARXIV_OUT}
	git archive --format=tar HEAD: | (cd ${ARXIV_OUT}; tar xf -)
	(cd ${ARXIV_OUT}; rm ${ARXIV_REMOVED}; cp ../article.bbl article.bbl; tar cvzf arxiv.tar.gz *; cp -i arxiv.tar.gz ../arxiv.tar.gz)

ci:
	git commit -m 'travail sur article-v2' .
	git push


==> strcat.tex <==



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "proxy-strcat"
%%% End:

